SwarmGear: Heterogeneous Swarm of Drones with Reconfigurable Leader Drone and Virtual Impedance Links for Multi-Robot Inspection

The continuous monitoring by drone swarms remains a challenging problem due to the lack of power supply and the inability of drones to land on uneven surfaces. Heterogeneous swarms, including ground and aerial vehicles, can support longer inspections and carry a higher number of sensors on board. However, their capabilities are limited by the mobility of wheeled and legged robots in a cluttered environment. In this paper, we propose a novel concept for autonomous inspection that we call SwarmGear. SwarmGear utilizes a heterogeneous swarm that investigates the environment in a leader-follower formation. The leader drone is able to land on rough terrain and traverse it by four compliant robotic legs, possessing both the functionalities of an aerial and mobile robot. To preserve the formation of the swarm during its motion, virtual impedance links were developed between the leader and the follower drones. We evaluated experimentally the accuracy of the hybrid leader drone's ground locomotion. By changing the step parameters, the optimal step configuration was found. Two types of gaits were evaluated. The experiments revealed low crosstrack error (mean of 2 cm and max of 4.8 cm) and the ability of the leader drone to move with a 190 mm step length and a 3 degree standard yaw deviation. Four types of drone formations were considered. The best formation was used for experiments with SwarmGear, and it showed low overall crosstrack error for the swarm (mean 7.9 cm for the type 1 gait and 5.1 cm for the type 2 gait). The proposed system can potentially improve the performance of autonomous swarms in cluttered and unstructured environments by allowing all agents of the swarm to switch between aerial and ground formations to overcome various obstacles and perform missions over a large area.

==> Draft.tex <==
% A two-part experiment was carried out to evaluate the proposed approach of swarm landing: landing on a static mobile robot and landing on a moving mobile robot moving with different velocities. At the start of each experiment, the platform is located at 2 m distance from the swarm, and the leader drone tries to find the target with the rest of the swarm following it. While in moving condition, and the swarm tries to land on it. The swarm of drones used for the experiment includes one leader drone, which weighs 0.262 kg, including 450 mAh 3S battery and the other drones which weighs 0.032 kg including 240 mAh 1S battery. The on-Board processor used for the leader drone is Crazyflie 2.1 firmware with a big quad deck extension and Raspberry Pi 4 with a Pi camera which provides 640x480 RGB images at a rate of 30 fps to the target detection module, whereas the rest of the swarm consists of only the Crazyflie 2.1 controller.
